Hide & Seek: Transformer Symmetries Obscure Sharpness & Riemannian Geometry Finds It

The concept of sharpness has been successfully applied to traditional architectures like MLPs and CNNs to predict their generalization. For transformers, however, recent work reported weak correlation between flatness and generalization. We argue that existing sharpness measures fail for transformers, because they have much richer symmetries in their attention mechanism that induce directions in parameter space along which the network or its loss remain identical. We posit that sharpness must account fully for these symmetries, and thus we redefine it on a quotient manifold that results from quotienting out the transformer symmetries, thereby removing their ambiguities. Leveraging tools from Riemannian geometry, we propose a fully general notion of sharpness, in terms of a geodesic ball on the symmetry-corrected quotient manifold. In practice, we need to resort to approximating the geodesics. Doing so up to first order yields existing adaptive sharpness measures, and we demonstrate that including higher-order terms is crucial to recover correlation with generalization. We present results on diagonal networks with synthetic data, and show that our geodesic sharpness reveals strong correlation for real-world transformers on both text and image classification tasks.

==> preamble/neurips.tex <==
% copied from icml.tex, then added stuff from neurips_2024.tex




% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2024


% ready for submission
%\usepackage{neurips_2024}


% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
%     \usepackage[preprint]{neurips_2024}


% to compile a camera-ready version, add the [final] option, e.g.:
%     \usepackage[final]{neurips_2024}


% to avoid loading the natbib package, add option nonatbib:
%    \usepackage[nonatbib]{neurips_2024}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
% \usepackage{subfigure} % we use the `subfigure' environment `subcaption' package instead
\usepackage{booktabs} % for professional tables

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2024} with \usepackage[nohyperref]{icml2024} above.
\usepackage{hyperref} % hyperlinks

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:

% \usepackage[accepted]{icml2025}

% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{example}[theorem]{Example}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:



\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{amsfonts}       % blackboard math symbols



==> sections/additional_analysis_kunin.tex <==
The Hessian is often approximated through other quantities, such as the
GGN/Fisher or the empirical Fisher and we want to better understand whether
these proxies are constrained in the same way as the Hessian, or differently.

\fd{We could also look at other objects that people care about, like the
  empirical NTK.}

\subsubsection{Model Jacobian}
\label{sec:model-jacobian}
Approximations of the Hessian almost always use the model's Jacobian. Let $f:
\sR^D \times \sR^C: \vtheta \mapsto f(\vtheta)$ denote the neural network's
$C$-dimensional output. We can imagine $f$ to consist of components $f_1, \dots,
f_C$. If $f$ is invariant under an action $\psi$ of a continuous group, then the
same constraints as in \Cref{sec:background} hold, but \emph{for each component
  of $f$}. We will now translate the gradient constraints and express them in
terms of the model's Jacobian $\left.\mJ f \right\rvert_{\vtheta} =
(\left.\nabla f_1 \right\rvert_{\vtheta}, \dots, \left.\nabla f_C
\right\rvert_{\vtheta}) \in \sR^{C \times D}$.

\paragraph{Translation symmetry:} \fd{TODO}

\paragraph{Scale symmetry:} \fd{TODO}

\paragraph{Re-scale symmetry:} \fd{TODO}

\subsubsection{Popular curvature approximations}
Here, we define the Hessian, GGN, and empirical Fisher on a data set (or mini-batch).
\begin{align}
  \mH = \text{\fd{(TODO Define Hessian)}}
  \\
  \mG = \text{\fd{(TODO Define GGN/Fisher)}}
  \\
  \mK = \text{\fd{(TODO Define empirical Fisher)}}
\end{align}
Based on the model Jacobian's constraints from \Cref{sec:model-jacobian}, we can
make the following connections between $\mH$ and its common approximations $\mG,
\mK$:
\begin{itemize}
\item Translation symmetry
  \begin{align*}
    \mG \vone_{\sA} = \mK \vone_{\sA} = \mH \vone_{\sA} = \vzero
  \end{align*}

\item Scale symmetry

\item Re-scale symmetry
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/background.tex <==
\paragraph{Setting:} We consider a neural network $f: \sR^D \times \sR^M \to
\sR^C, (\vtheta, \vx) \mapsto \vf := f(\vtheta, \vx) $ which maps an input $\vx$
to a prediction $\vf$ using parameters $\vtheta$, and its cost function $c:
\sR^C \times \sR^C \to \sR: (\vf, \vy) \mapsto c(\vf, \vy)$. (forget about this
for now, but it might be relevant for introducing the other deep learning
quantities at a later stage.) In the following, we restrict the analysis to the
parameter space, focusing on data-independent symmetries.

Therefore, we consider $f: \sR^D \to \sR^C, \vtheta \mapsto f(\vtheta)$, and the
loss $\ell: \sR^D \to \sR, \vtheta \mapsto \ell(\vtheta) = c(f(\vtheta))$.

\subsection{Constraints Imposed by a Continuous Symmetry}

We consider continuous symmetries of the loss $\ell$. Let $\gG$ denote the
symmetry group and $\vpsi: \sR^D \times \gG \to \sR^D: (\vtheta, \alpha) \mapsto
\vpsi(\vtheta, \alpha)$ denote its action on the parameter space. The loss is
symmetric under $\gG$ if $\ell(\vtheta) = \ell(\vpsi(\vtheta, \alpha))\ \forall\
\vtheta \in \sR^D, \alpha \in \gG$. For the derivative functions below, it will
be sufficient to think of $\alpha$ as a scalar.

\paragraph{General constraints (\citet{kunin2021symmetry}):} By analysis of the
augmented function $\tilde{\ell}(\vtheta, \alpha) = \ell(\vpsi(\vtheta,
\alpha))$,~\cite{kunin2021symmetry} derive different constraints that symmetry
imposes on the gradient and Hessian of $\ell$ under a group action. For the
gradient, we obtain (using functional notation)
\begin{align}
  \partial_{(\vtheta, \alpha)} \tilde{\ell}
  =
  \begin{pmatrix}
    \partial_{\vtheta}\tilde{\ell}
    \\
    \partial_{\alpha}\tilde{\ell}
  \end{pmatrix}
  =
  \begin{pmatrix}
    \partial_{\vtheta}\vpsi
    \partial_{\vpsi}\tilde{\ell}
    \\
    \partial_{\vpsi} \tilde{\ell}
    \partial_{\alpha}\vpsi
  \end{pmatrix}
  =
  \begin{pmatrix}
    \partial_{\vtheta}\ell
    \\
    0
  \end{pmatrix}\,.
\end{align}
For the Hessian, one obtains (using functional notation)
\begin{align}
  \begin{split}
    \partial^2_{(\vtheta, \alpha)} \tilde{\ell}
    =
    \begin{pmatrix}
      \partial^2_{\vtheta} \tilde{\ell}
      &
        \partial_{\vtheta}\partial_{\alpha} \tilde{\ell}
      \\
      \partial_{\alpha}\partial_{\vtheta} \tilde{\ell}
      &
        \partial^2_{\alpha} \tilde{\ell}
    \end{pmatrix}
    &=
      \begin{pmatrix}
        \partial_{\vtheta}^2 \vpsi \partial_{\vpsi}\tilde{\ell}
        +
        \partial_{\vtheta}\vpsi \partial_{\vtheta}\vpsi \partial_{\vpsi}^2 \tilde{\ell}
        &
          \partial_{\vtheta}\partial_{\alpha}\vpsi \partial_{\vpsi}\tilde{\ell}
          +
          \partial_{\alpha}\vpsi \partial_{\vtheta}\vpsi \partial_{\vpsi}^2 \tilde{\ell}
        \\
        \partial_{\alpha}\partial_{\vtheta}\vpsi \partial_{\vpsi}\tilde{\ell}
        +
        \partial_{\vtheta}\vpsi \partial_{\alpha} \vpsi \partial_{\vpsi}^2\tilde{\ell}
        &
          \partial_{\alpha}^2\vpsi \partial_{\vpsi}\tilde{\ell}
          +
          \partial_{\alpha}\vpsi \partial_{\alpha}\vpsi \partial_{\vpsi}^2\tilde{\ell}
      \end{pmatrix}
    \\
      &=
        \begin{pmatrix}
          \partial_{\vtheta}\ell & 0
          \\
          0 & 0
        \end{pmatrix}\,.
  \end{split}
\end{align}

In gradient and Jacobian notation, for any $(\vtheta, \alpha)$, we get the
gradient constraints
\begin{subequations}
  \label{eq:general-gradient-constraints}
  \begin{align}
    \left.
    \nabla \ell
    \right\rvert_{\vpsi(\vtheta,\alpha)}
    &=
      \left.\left(
      \mJ_{\vtheta}\vpsi
      \right)^{\top}  \right\rvert_{(\vtheta, \alpha)}
      \left.
      \nabla \ell
      \right\rvert_{\vtheta}\,,
    \\
    \left\langle
    \left. \nabla \ell \right\rvert_{\vpsi(\vtheta,\alpha)},
    \left.
    \left(
    \mJ_{\alpha}\vpsi
    \right)
    \right\rvert_{(\vtheta, \alpha)}
    \right\rangle
    &=
      0\,.
  \end{align}
\end{subequations}
In gradient and Jacobian notation, for any $(\vtheta, \alpha)$ we get the
Hessian constraints
\begin{subequations}
  \label{eq:general-hessian-constraints}
  \begin{align}
    \sum_{i=1}^{D}
    \left.
    \nabla_{\vtheta}^2 [\vpsi]_i
    \right\rvert_{(\vtheta, \alpha)}
    \left.
    \left[
    \nabla \ell
    \right]_i
    \right\rvert_{\vpsi(\vtheta,\alpha)}
    +
    \left.
    \left(
    \mJ_{\vtheta} \vpsi
    \right)^{\top}
    \right\rvert_{(\vtheta, \alpha)}
    \left.
    \nabla^2 \ell
    \right\rvert_{\vpsi(\vtheta,\alpha)}
    \left.
    \left(
    \mJ_{\vtheta} \vpsi
    \right)
    \right\rvert_{(\vtheta, \alpha)}
    &=
      \left.
      \nabla^2\ell
      \right\rvert_{\vtheta}\,,
    \\
    \left.
    \left(
    \mJ_{\vtheta}
    \left(
    \mJ_{\alpha}\vpsi
    \right)
    \right)^{\top}
    \right\rvert_{(\vtheta, \alpha)}
    \left.
    \nabla \ell
    \right\rvert_{\vpsi(\vtheta, \alpha)}
    +
    \left.
    \left(
    \mJ_{\alpha} \vpsi
    \right)^{\top}
    \right\rvert_{(\vtheta, \alpha)}
    \left.
    \nabla^2 \ell
    \right\rvert_{\vpsi(\vtheta, \alpha)}
    \left.
    \left(
    \mJ_{\vtheta} \vpsi
    \right)
    \right\rvert_{(\vtheta, \alpha)}
    &=
      0\,,
    \\
    \sum_{i=1}^D
    \left.
    \nabla_{\alpha}^2 [\vpsi]_i
    \right\rvert_{(\vtheta, \alpha)}
    \left.
    \left[
    \nabla \ell
    \right]_i
    \right\rvert_{\vpsi(\vtheta, \alpha)}
    +
    \left.
    \left(
    \mJ_{\alpha} \vpsi
    \right)^{\top}
    \right\rvert_{(\vtheta, \alpha)}
    \left.
    \nabla^2 \ell
    \right\rvert_{\vpsi(\vtheta, \alpha)}
    \left.
    \left(
    \mJ_{\alpha} \vpsi
    \right)
    \right\rvert_{(\vtheta, \alpha)}\,.
  \end{align}
\end{subequations}

\paragraph{Local constraints (\citet{kunin2021symmetry}):} The relevant case
for us are the constraints when we set $\alpha$ to the group's identity element
$e$, since in this case applying the group action does not move us in parameter
space, $\vpsi(\vtheta, e) = \vtheta$.

Evaluating \Cref{eq:general-gradient-constraints} at the identity element, we
get the following local gradient constraints:
\begin{subequations}
  \label{eq:local-gradient-constraints}
  \begin{align}
    \left.
    \nabla \ell
    \right\rvert_{\vtheta}
    &=
      \left.\left(
      \mJ_{\vtheta}\vpsi
      \right)^{\top}  \right\rvert_{(\vtheta, \alpha=e)}
      \left.
      \nabla \ell
      \right\rvert_{\vtheta}\,,
      \qquad
      \implies
      \left.\left(
      \mJ_{\vtheta}\vpsi
      \right)^{\top}  \right\rvert_{(\vtheta, \alpha=e)}
      = \mI
    \\
    \left\langle
    \left. \nabla \ell \right\rvert_{\vtheta},
    \left.
    \left(
    \mJ_{\alpha}\vpsi
    \right)
    \right\rvert_{(\vtheta, \alpha=e)}
    \right\rangle
    &=
      0\,.
  \end{align}
\end{subequations}
Evaluating \Cref{eq:general-hessian-constraints} at the identity element, we get
the following local Hessian constraints (also, using that the group action's
Jacobian w.r.t. $\vtheta$ evaluates to the identity matrix at $\alpha=e$
from \Cref{eq:local-gradient-constraints}):
\begin{subequations}
  \label{eq:local-hessian-constraints}
  \begin{align}
    \sum_{i=1}^{D}
    \left.
    \nabla_{\vtheta}^2 [\vpsi]_i
    \right\rvert_{(\vtheta, \alpha=e)}
    \left.
    \left[
    \nabla \ell
    \right]_i
    \right\rvert_{\vtheta}
    +
    \left.
    \nabla^2 \ell
    \right\rvert_{\vtheta}
    &=
      \left.
      \nabla^2\ell
      \right\rvert_{\vtheta}\,,
    \\
    \left.
    \left(
    \mJ_{\vtheta}
    \left(
    \mJ_{\alpha}\vpsi
    \right)
    \right)^{\top}
    \right\rvert_{(\vtheta, \alpha=e)}
    \left.
    \nabla \ell
    \right\rvert_{\vtheta}
    +
    \left.
    \left(
    \mJ_{\alpha} \vpsi
    \right)^{\top}
    \right\rvert_{(\vtheta, \alpha=e)}
    \left.
    \nabla^2 \ell
    \right\rvert_{\vtheta}
    &=
      0\,,
    \\
    \sum_{i=1}^D
    \left.
    \nabla_{\alpha}^2 [\vpsi]_i
    \right\rvert_{(\vtheta, \alpha=e)}
    \left.
    \left[
    \nabla \ell
    \right]_i
    \right\rvert_{\vtheta}
    +
    \left.
    \left(
    \mJ_{\alpha} \vpsi
    \right)^{\top}
    \right\rvert_{(\vtheta, \alpha=e)}
    \left.
    \nabla^2 \ell
    \right\rvert_{\vtheta}
    \left.
    \left(
    \mJ_{\alpha} \vpsi
    \right)
    \right\rvert_{(\vtheta, \alpha=e)}
    &=
      0\,.
  \end{align}
\end{subequations}

\subsection{Common Continuous Symmetries in Deep Learning}

\citet{kunin2021symmetry} mentions three important symmetries, (i) translation,
(ii) scale, and (iii) re-scale. The associated constraints are given in tables
in the appendix. We list these results here.

\paragraph{Translation symmetry:} If we can shift a parameter subset by the
same value $\alpha \in \sR$ without changing the loss, it is invariant under
translation. The symmetry group is $\gG = (\sR, +)$ and the group action is
\begin{align*}
  \vpsi(\vtheta, \alpha) = \vtheta + \alpha \vone_{\sA}\,,
\end{align*}
where $\sA$ is a parameter space mask that restricts the shift by $\alpha$ to
the relevant subspace.

The group action's derivatives are
\begin{align*}
  \left.
  \left(
  \mJ_{\alpha} \vpsi
  \right)
  \right\rvert_{(\vtheta, \alpha)}
  =
  \vone_{\sA}\,,
  \qquad
  \left.
  \left(
  \mJ_{\vtheta} \vpsi
  \right)
  \right\rvert_{(\vtheta, \alpha)}
  =
  \mI\,,
  \qquad
  \partial_{\alpha}^2\vpsi
  =
  \partial_{\vtheta}^2\vpsi
  =
  \partial_{\alpha}\partial_{\vtheta} \vpsi
  =
  0\,.
\end{align*}
For the general gradient constraints \Cref{eq:general-gradient-constraints}, we get
\begin{subequations}
  \begin{align}
    \left.
    \nabla \ell
    \right\rvert_{\vpsi(\vtheta,\alpha)}
    &=
      \left.
      \nabla \ell
      \right\rvert_{\vtheta}\,,
    \\
    \left\langle
    \left. \nabla \ell \right\rvert_{\vpsi(\vtheta,\alpha)},
    \vone_{\sA}
    \right\rangle
    &=
      0
      \qquad \Leftrightarrow \qquad
      \left\langle
      \left.
      \left[
      \nabla \ell
      \right]_{\sA}
      \right\rvert_{\vpsi(\vtheta,\alpha)},
      \vone
      \right\rangle
      =
      0\,.
  \end{align}
  The general Hessian constraints \Cref{eq:general-hessian-constraints} simplify
  to (omitting the trivial equalities)
  \begin{align}
    \left.
    \nabla^2 \ell
    \right\rvert_{\vpsi(\vtheta, \alpha)}
    \vone_{\sA}
    &=
      \vzero
      \qquad \Leftrightarrow \qquad
      \left.
      \left[
      \nabla^2 \ell
      \right]_{\sA, \sA}
      \right\rvert_{\vpsi(\vtheta, \alpha)}
      \vone
      = \vzero
      \,.
  \end{align}
\end{subequations}
The local constraints
\Cref{eq:local-gradient-constraints,eq:local-hessian-constraints} reduce to
\begin{subequations}
  \begin{align}
    \left\langle
    \left. \nabla \ell \right\rvert_{\vtheta},
    \vone_{\sA}
    \right\rangle
    &=
      0
      \qquad \Leftrightarrow \qquad
      \left\langle
      \left.
      \left[
      \nabla \ell
      \right]_{\sA}
      \right\rvert_{\vtheta},
      \vone
      \right\rangle
      =
      0\,,
    \\
    \left.
    \nabla^2 \ell
    \right\rvert_{\vtheta}
    \vone_{\sA}
    &=
      \vzero
      \qquad \Leftrightarrow \qquad
      \left.
      \left[
      \nabla^2 \ell
      \right]_{\sA, \sA}
      \right\rvert_{\vtheta}
      \vone
      = \vzero
      \,.
  \end{align}
\end{subequations}
The vector of ones is orthogonal to the $\sA$-restricted gradient and in the
$\sA$-restricted Hessian's kernel.

{%
  \color{blue} This is a very weak hint, but if you use the gradient outer
  product $\nabla \ell \left( \nabla \ell \right)^{\top}$ as a curvature proxy
  for the translation-invariant parameters, its kernel also includes the vector
  of ones, i.e. $\nabla \ell \left( \nabla \ell \right)^{\top} \vone = \left(
    \nabla^2 \ell \right) \vone = \vzero$.
  %
}

\paragraph{Scale symmetry:} If we can scale a parameter subset by a positive
value $\alpha > 0$ without changing the loss, it is scale-invariant. The
symmetry group is $\gG = (\sR^+, \cdot) := GL^+_1(\sR)$ and the group action is
\begin{align*}
  \vpsi(\vtheta, \alpha)
  =
  \left(
  \alpha_{\sA}
  +
  \vone_{\overline{\sA}}
  \right)
  \odot
  \vtheta\,,
\end{align*}
where $\sA$ is a parameter mask and $\overline{\sA}$ its complement.

The group action's derivatives are
\begin{align*}
  \left.
  \left(
  \mJ_{\alpha} \vpsi
  \right)
  \right\rvert_{(\vtheta, \alpha)}
  &=
    \vone_{\sA} \odot \vtheta
    :=
    \vtheta_{\sA}\,,
    \qquad
    \left.
    \left(
    \mJ_{\vtheta} \vpsi
    \right)
    \right\rvert_{(\vtheta, \alpha)}
    =
    \diag \left(
    \alpha_{\sA} + \vone_{\overline{\sA}}
    \right)\,,
  \\
  \left.
  \left(
  \mJ_{\vtheta}
  \left(
  \mJ_{\alpha}\vpsi
  \right)
  \right)
  \right\rvert_{(\vtheta, \alpha)}
  &=
    \diag \left(
    \vone_{\sA}
    \right)\,,
    \qquad
    \partial_{\vtheta}^2\vpsi
    =
    \partial_{\alpha}^2 \vpsi
    = 0\,.
\end{align*}
For the general constraints
\Cref{eq:general-gradient-constraints,eq:general-hessian-constraints}, we obtain
(omitting the trivial equalities)
\begin{align}
  TODO
\end{align}
The local constraints
\Cref{eq:local-gradient-constraints,eq:local-hessian-constraints} reduce to
\begin{subequations} \label{eq:scaling-constraints}
  \begin{align}
    \left\langle
    \left.
    \nabla \ell
    \right\rvert_{\vtheta},
    \vtheta_{\sA}
    \right\rangle
    = 0
    \qquad
    &\Leftrightarrow
      \qquad
      \left\langle
      \left.
      \left[
      \nabla \ell
      \right]_{\sA}
      \right\rvert_{\vtheta},
      \left[
      \vtheta
      \right]_{\sA}
      \right\rangle
      = 0\,,
    \\
    \left.
    \nabla^2 \ell
    \right\rvert_{\vtheta}
    \vtheta_{\sA}
    +
    \left.
    \nabla \ell
    \right\rvert_{\vtheta} \odot \vone_{\sA}
    =
    \vzero
    \qquad
    &\Leftrightarrow
      \qquad
      \left.
      \left[
      \nabla^2 \ell
      \right]_{\sA,\sA}
      \right\rvert_{\vtheta}
      \left[
      \vtheta
      \right]_{\sA}
      +
      \left.
      \left[
      \nabla \ell
      \right]_{\sA}
      \right\rvert_{\vtheta}
      =
      \vzero\,,
    \\
    \vtheta_{\sA}^{\top}
    \left(
    \left.
    \nabla^2\ell
    \right\rvert_{\vtheta}
    \right)
    \vtheta_{\sA}
    = 0
    \qquad
    &\Leftrightarrow
      \qquad
      \left[
      \vtheta
      \right]_{\sA}^{\top}
      \left.
      \left[
      \nabla^2\ell
      \right]_{\sA, \sA}
      \right\rvert_{\vtheta}
      \left[
      \vtheta
      \right]_{\sA}
      = 0\,.
  \end{align}
\end{subequations}

%
{%
  \color{blue}

  The second equation let us compute Newton steps for free if we restrict the
  Hessian to the subspace indicated by $\sA$ (common in practice to reduce
  computation). The Newton step is simply given by the current parameter value.
  This is a good motivation why symmetry may be useful to speed up computation.
  Instead of computing first- and second-order derivatives, then solving a
  linear system (adds a lot of computation), we can instead take the current
  parameters (zero cost). Remarks:
  \begin{itemize}
  \item This Newton step would even be \emph{cheaper} than gradient descent as
    we don't need to perform a forward+backward pass.

  \item The second equation above holds for \emph{any data}. Hence, the Newton
    step does not suffer from noise from mini-batching. This is promising for
    second-order methods in this subspace, as their performance usually suffers
    from noisy observations of the gradient and Hessian.
  \end{itemize}

  Just like for translation symmetry, we see that if we use the gradient outer
  product as proxy for the Hessian, then this curvature proxy satisfies the
  third constraint due to the first equation (however, it does not satisfy the
  second equation).
  %
}

\paragraph{Rescale symmetry:} If we can scale a parameter subset by a positive
scalar $\alpha > 0$ and at the same time another subset by $\frac{1}{\alpha}$
without changing the loss, it is rescale-invariant. The symmetry group is $\gG =
(\sR, \cdot) := GL^+_1(\sR)$ with action
\begin{align*}
  \vpsi(\vtheta, \alpha) =
  \alpha_{\sA_1} \oslash \alpha_{\sA_2}
  \odot
  \vtheta
\end{align*}
where $\sA_1, \sA_2$ are two disjoint masks.

The group action's derivatives are
\begin{align*}
  \left.
  \left(
  \mJ_{\alpha} \vpsi
  \right)
  \right\rvert_{(\vtheta, \alpha)}
  &=
    \vtheta_{\sA_1} - \frac{1}{\alpha^2} \vtheta_{\sA_2}\,,
    \qquad
    \left.
    \left(
    \mJ_{\vtheta} \vpsi
    \right)
    \right\rvert_{(\vtheta, \alpha)}
    =
    \diag \left(
    \alpha_{\sA_1} \oslash \alpha_{\sA_2}
    \right)\,,
  \\
  \left.
  \left(
  \mJ_{\vtheta}
  \left(
  \mJ_{\alpha}\vpsi
  \right)
  \right)
  \right\rvert_{(\vtheta, \alpha)}
  &=
    \diag \left(
    \vone_{\sA_1} - \frac{1}{\alpha^2} \vone_{\sA_2}
    \right)\,,
    \qquad
    \left.
    \nabla_{\alpha}^2
    \left[
    \vpsi
    \right]_i
    \right\rvert_{(\vtheta, \alpha)}
    =
    \frac{2}{\alpha^3}
    \left[
    \vtheta
    \right]_i
    \quad (i \in \sA_2)
    \,,
  \\
  \partial_{\vtheta}^2\vpsi
  &= 0\,.
\end{align*}
The general constraints
\Cref{eq:general-gradient-constraints,eq:general-hessian-constraints} translate
into (omitting the trivial equalities)
\begin{align}
  TODO
\end{align}
The local constraints
\Cref{eq:local-gradient-constraints,eq:local-hessian-constraints} reduce to
\begin{subequations}
  \begin{align}
    \begin{split}
      \left\langle
      \left.
      \nabla \ell
      \right\rvert_{\vtheta},
      \vtheta_{\sA_1}
      -
      \vtheta_{\sA_2}
      \right\rangle
      = 0
      \\
      \Leftrightarrow\qquad
      \left\langle
      \left.
      \left[
      \nabla \ell
      \right]_{\sA_1}
      \right\rvert_{\vtheta},
      \left[
      \vtheta
      \right]_{\sA_1}
      \right\rangle
      =
      \left\langle
      \left.
      \left[
      \nabla \ell
      \right]_{\sA_2}
      \right\rvert_{\vtheta},
      \left[
      \vtheta
      \right]_{\sA_2}
      \right\rangle\,,
    \end{split}
    \\
    \begin{split}
      \left.
      \nabla^2 \ell
      \right\rvert_{\vtheta}
      \left(
      \vtheta_{\sA_1}
      -
      \vtheta_{\sA_2}
      \right)
      +
      \left.
      \nabla \ell
      \right\rvert_{\vtheta}
      \odot
      \left(
      \vone_{\sA_1}
      -
      \vone_{\sA_2}
      \right)
      =
      \vzero
      \\
      \Leftrightarrow
      \qquad
      \left.
      \left[
      \nabla^2 \ell
      \right]_{\sA_1 \cup \sA_2,\sA_1\cup\sA_2}
      \right\rvert_{\vtheta}
      \begin{pmatrix}
        \left[
        \vtheta
        \right]_{\sA_1}
        \\
        -
        \left[
        \vtheta
        \right]_{\sA_2}
      \end{pmatrix}
      +
      \begin{pmatrix}
        \left.
        \left[
        \nabla \ell
        \right]_{\sA_1}
        \right\rvert_{\vtheta}
        \\
        - \left.
        \left[
        \nabla \ell
        \right]_{\sA_2}
        \right\rvert_{\vtheta}
      \end{pmatrix}
      =
      \vzero\,,
    \end{split}
    \\
    \begin{split}
      \left(
      \vtheta_{\sA_1}
      -
      \vtheta_{\sA_2}
      \right)
      ^{\top}
      \left(
      \left.
      \nabla^2\ell
      \right\rvert_{\vtheta}
      \right)
      \left(
      \vtheta_{\sA_1}
      -
      \vtheta_{\sA_2}
      \right)
      +
      \left\langle
      \left.
      \nabla \ell
      \right\rvert_{\vtheta},
      2 \vtheta_{\sA_2}
      \right\rangle
      = 0
      \\
      \Leftrightarrow
      \qquad
      \begin{pmatrix}
        \left[
        \vtheta
        \right]_{\sA_1}
        \\
        - \left[
        \vtheta
        \right]_{\sA_2}
      \end{pmatrix}^{\top}
      \left.
      \left[
      \nabla^2\ell
      \right]_{\sA_1\cup \sA_2, \sA_1\cup\sA_2}
      \right\rvert_{\vtheta}
      \begin{pmatrix}
        \left[
        \vtheta
        \right]_{\sA_1}
        \\
        - \left[
        \vtheta
        \right]_{\sA_2}
      \end{pmatrix}
      +
      2
      \left\langle
      \left.
      \left[ \nabla \ell\right]_{\sA_2}
      \right\rvert_{\vtheta},
      \left[
      \vtheta
      \right]_{\sA_2}
      \right\rangle
      = 0\,.
    \end{split}
  \end{align}
\end{subequations}
{%
  \color{blue}

  Note: The third equation differs from \cite{kunin2021symmetry}. Could be a
  mistake of mine, or the paper (the result is not further used there).

  %
}

\subsection{Examples for Continuous Symmetries in Deep Neural Networks}

The general recipe is as follows: If we have an operation with a specific
symmetry w.r.t.\ its input, and a linear layer preceding that operation, the
symmetry translates onto the parameters of that layer.

\subsubsection{Translation symmetry}
\label{subsec:examples-translation-symmetry}
\paragraph{Softmax:} The $\softmax$ function is invariant under translations,
$\softmax(\vx + \alpha \vone) = \softmax(\vx)$.

If we feed the output into a linear layer into a $\softmax$, this imposes
translation invariance\dots
\begin{itemize}
\item \dots of the bias under the group action $\vpsi: \vb \mapsto \vb + \alpha
  \vone$: $\softmax(\mW \vx + \vb + \alpha \vone) = \softmax(\mW \vx + \vb)$.
\item \dots of each column $j$ of the weight matrix under the group action
  $\vpsi: \left[ \mW \right]_{:,j} \mapsto \left[ \mW \right]_{:,j} + c$:
  $\softmax( \mW \vx + c \sum_{i} \ve_i \ve_j^{\top}\vx + \vb) = \softmax( \mW
  \vx + \underbrace{\ve_j^{\top}\vx}_{\alpha} \sum_{i} \ve_i + \vb) = \softmax(
  \mW \vx + \alpha \vone + \vb) = \softmax( \mW \vx + \vb)$.
\item Since all actions are linear, we can compose them and shift different
  weight matrix columns and the bias vector at the same time.
\end{itemize}

{%
  \color{blue}%

  The attention layer applies $\softmax$ over a scaled version of $\mQ
  \mK^{\top}$. It would be interesting to write down the translation symmetry
  for its parameters here.
  %
}

\paragraph{Batch normalization (BN):} BN \cite{ioffe2015batch} in train mode is
invariant when all elements across a batch dimension are shifted by the same
amount: For a batch of vectors $\{ \vx_1, \dots, \vx_N\}$ and a vector $\valpha$
with arbitrary elements, we have $\batchnorm(\{ \vx_1, \dots, \vx_N\})
= \batchnorm(\{ \valpha + \vx_1, \dots, \valpha + \vx_N\})$.

\begin{itemize}
\item This is why popular architectures like ResNet18 with \texttt{Conv2d} $\to$
  \texttt{BatchNorm} blocks disable the bias term for convolutions. Adding a
  bias would simply shift the input to BN by a constant vector and leave its
  output unchanged (mentioned in \cite[Section 3.2]{ioffe2015batch}).
\end{itemize}

We can break this further down into components: Pick a component $i$ and an
$\alpha \in \sR$. Then, the translation $\left[ \vx_n \right]_i \to \left[ \vx_n
\right]_i + \alpha\,, \ n = 1, \dots, N$ leaves BN unchanged.

\subsubsection{Scale symmetry}

\paragraph{Batch normalization (BN):} BN \cite{ioffe2015batch} in train mode is
\textbf{approximately} scale-invariant (exactly for $\epsilon = 0$) w.r.t. its
input: If we scale a single component of the input across the batch dimension by
a positive scalar, the output of BN remains unchanged. For a linear layer
preceding BN, this imposes scale-invariance on the parameters.

For a batch of vectors $\{ \vx_1, \dots, \vx_N\}$ and a vector $\valpha$ with
arbitrary positive elements,
\begin{align*}
  \batchnorm(\{ \vx_1, \dots, \vx_N\})
  =
  \batchnorm(\{ \valpha \odot \vx_1, \dots, \valpha \odot \vx_N\})\,.
\end{align*}
(This includes the special case $\valpha = \alpha \vone$ from
\cite{kunin2021symmetry}, which is also mentioned in \cite[Section
3.3]{ioffe2015batch}). It is easy to see from its definition
\begin{align*}
  \left[
  \batchnorm(\{ \vx_1, \dots, \vx_N\})
  \right]_{n,i}
  &=
    \frac{
    \left[ \vx_n \right]_i - \left[ \vmu \right]_i
    }{
    \sqrt{
    \left[ \vsigma \right]_i^2 + \epsilon
    }}
    \left[ \vgamma \right]_i
    +
    \left[ \vbeta \right]_i
    \shortintertext{where}
    \left[ \vmu \right]_i
  &=
    \frac{1}{N} \sum_n \left[ \vx_n \right]_i
  \\
  \left[ \vsigma \right]_i^2
  &=
    \frac{1}{N} \sum_n
    \left(
    \left[ \vx_n \right]_i
    -
    \left[ \vmu \right]_i
    \right)^2
\end{align*}
Under the group action $\{ \vx_1, \dots, \vx_N \} \to \{ \valpha \vx_1, \dots,
\valpha \vx_N \}$, we have
\begin{align*}
  \left[ \vmu \right]_i
  &\to
    \left[ \valpha \right]_i \left[ \vmu \right]_i
  \\
  \left[ \vsigma \right]_i^2
  &\to
    \left[ \valpha \right]_i^2 \left[ \vsigma \right]_i^2
    \shortintertext{and}
    \left[
    \batchnorm(\{ \vx_1, \dots, \vx_N\})
    \right]_{n,i}
  &\to
    \frac{
    \left[ \vx_n \right]_i - \left[ \vmu \right]_i
    }{
    \sqrt{
    \left[ \vsigma \right]_i^2 + \frac{\epsilon}{\left[ \vsigma \right]_i^2}
    }}
    \approx
    \left[
    \batchnorm(\{ \vx_1, \dots, \vx_N\})
    \right]_{n,i}
\end{align*}
Note that exact scale-invariance only holds if $\epsilon = 0$.

This translates into symmetries of parameters in a preceding linear layer as
follows: Consider a linear layer preceding BN (without biases as they don't
matter, see BN discussion in \Cref{subsec:examples-translation-symmetry}),
$\batchnorm(\{ \mW \vx_1, \dots, \mW \vx_N\})$. The properties of BN impose
scale invariance\dots
\begin{itemize}
\item \dots of the $j$-th row of the weight matrix under the group action
  $\vpsi: \left[ \mW \right]_{j, :} \mapsto \alpha \left[ \mW \right]_{j, :}$.
  This action effectively scales the $j$-th component of the input to BN.
\end{itemize}
A special case is re-scaling all rows at once by the same scalar. For
convolutions, this corresponds to multiplying the kernel by that scalar.

{%
  \color{blue}

  Other normalization layers (for instance layer norm, group norm) probably
  impose a similar scale symmetry. It would be interesting to document these
  here.
  %

  \paragraph{Layer norm:} TODO

  \paragraph{Group norm:} TODO
}


\subsubsection{Re-scale symmetry}

\paragraph{Homogeneous element-wise functions:} A homogeneous function $\phi:
\sR \to \sR$ satisfies $\phi(z) = \phi'(z) z$. This includes ReLU, LeakyReLU,
and the identity. We will often write $\phi(\vz)$ for the element-wise
application of $\phi$ to the components of the vector $\vz$. Homogeneous
functions impose re-scale symmetry on the parameters before and after an
activated hidden unit. Consider $\mW^{(2)} \phi \left( \mW^{(1)} \vx + \vb^{(1)}
\right) + \vb^{(2)}$:
\begin{itemize}
\item This sub-network is re-scale invariant under the action $\vpsi:
  (\mW^{(1)}, \vb^{(1)}, \mW^{(2)}) \mapsto (\alpha\mW^{(1)}, \alpha\vb^{(1)},
  \frac{1}{\alpha}\mW^{(2)})$ with $\alpha > 0$, that is we can scale the
  preceding weights and bias term by $\alpha$, then re-scale the succeeding
  weights by $\frac{1}{\alpha}$.

\item On a more fine-grained level, we can scale a single row $j$ of $\mW^{(1)},
  \vb^{(1)}$, and apply the inverse scaling to the $j$-th column of $\mW^{(2)}$:
  \begin{align*}
    \vpsi:
    \begin{pmatrix}
      \left[ \mW^{(1)} \right]_{j,:}
      \\
      \left[ \vb^{(2)} \right]_j
      \\
      \left[
      \mW^{(2)}
      \right]_{:,j}
    \end{pmatrix}
    \mapsto
    \begin{pmatrix}
      \alpha \left[ \mW^{(1)}  \right]_{j, :}
      \\
      \alpha \left[ \vb^{(1)} \right]_j
      \\
      \frac{1}{\alpha} \left[ \mW^{(2)} \right]_{:,j}
    \end{pmatrix}\,.
  \end{align*}

\item We can compose multiple of the previous transformation to re-scale
  multiple rows/columns at the same time.

\item If the network is an alternating sequence of linear layers (with bias
  terms) and homogeneous transformations,
  \begin{align*}
    \phi^{(L)}\left(
    \mW^{(L)}
    \phi^{(L-1)}
    \left(
    \mW^{(L-1)}
    \phi^{(L-2)}\left(
    \dots
    \right)
    + \vb^{(L-1)}
    \right)
    + \vb^{(L)}
    \right)\,,
  \end{align*}
  we can pick $2$ layers $i_1, i_2$ with $i_2 > i_1$. By scaling the weights and
  biases of layers between $i_1$ and $i_2$, including $i_1$, and rescale the
  weights of layer $i_2$,
  \begin{align*}
    \mW^{(i)} &\mapsto \alpha \mW^{(i)}\,, \quad i = i_1, \dots, i_2 - 1\,,
    \\
    \vb^{(i)} &\mapsto \alpha \vb^{(i)}\,, \quad i = i_1, \dots, i_2 - 1\,,
    \\
    \mW^{(i_2)} &\mapsto \frac{1}{\alpha} \mW^{(i_2)}\,,
  \end{align*}
  this leaves the output unchanged.

\item We can compose multiple of the previous transformations with different
  choices for $\alpha > 0, i_1, i_2$. This symmetry is described in
  \cite{dinh2017sharp}.
  \begin{itemize}
  \item For illustration, ignore the bias terms. Then, we can pick $K$ layers
    $i_1, \dots, i_K$ and apply
    \begin{align*}
      \mW^{(i_k)} \mapsto \alpha_{i_k} \mW^{(i_k)}\,, \qquad k = 1, \dots, K
    \end{align*}
    subject to $\prod_{k=1}^K \alpha_{i_k} = 1$.
  \end{itemize}
\end{itemize}

\clearpage
\pagestyle{empty}
\begin{landscape}
  \section{Continuous Symmetries Cheatsheet}
  \begin{table}[htbp]
    \caption{Let $\ell: \sR^D \to \sR, \vtheta \mapsto \ell(\vtheta)$ be a loss
      function invariant under a symmetry group $\gG$ acting via an action
      $\vpsi: \sR^D \times \gG \to \sR^D, (\vtheta, \alpha) \mapsto
      \vpsi(\vtheta, \alpha)$. Let $\vone_{\sA}$ be a vector with ones in the
      positions indicated by the mask $\sA$. Let $\alpha_{\sA}:= \alpha
      \vone_{\sA} + \vone_{\overline{\sA}}$ be a vector with $\alpha$ in all
      entries indicated by the mask and zero otherwise. Let $\vtheta_{\sA}:=
      \vtheta \odot \vone_{\sA}$ be the masked parameter vector.}
    \begin{center}
      \begin{tabular}{lllll}
        \toprule
        \textbf{Symmetry}
        & \textbf{Action}
        & \textbf{Global constraints}
        & \textbf{Local constraints}
        & \textbf{Examples}
        \\
        \midrule
        \multirow{3}{*}{\textbf{Translation}}
        & \multirow{3}{*}{$\vpsi(\vtheta, \alpha) = \vtheta + \alpha_{\sA} \vone_{\sA}\,, \alpha \in \sR$}
        & TODO
        & TODO
        & Weights and bias before input to softmax
        \\
        &
        & TODO
        & TODO
        & Bias before input to BN in train mode
        \\
        &
        & TODO
        & TODO
        & TODO
        \\
        \multirow{3}{*}{\textbf{Scale}}
        & \multirow{3}{*}{$\vpsi(\vtheta, \alpha) = \alpha_{\sA} \odot \vtheta\,, \alpha > 0$}
        & TODO
        & TODO
        & TODO
        \\
        &
        & TODO
        & TODO
        & TODO
        \\
        &
        & TODO
        & TODO
        & TODO
        \\
        \multirow{3}{*}{\textbf{Re-scale}}
        & \multirow{3}{*}{$\vpsi(\vtheta, \alpha) = \alpha_{\sA_1} \oslash \alpha_{\sA_2} \odot \vtheta\,, \alpha > 0$}
        & TODO
        & TODO
        & TODO
        \\
        &
        & TODO
        & TODO
        & TODO
        \\
        &
        & TODO
        & TODO
        & TODO
        \\
        \bottomrule
      \end{tabular}
    \end{center}
  \end{table}
\end{landscape}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/conceptual_overview.tex <==
\subsection{Conceptual Overview}


\fd{Do a pass to make sure flow makes sense and all objects of the figure are explained.}
We first provide an informal and intuitive description of our approach and of all objects involved.
See \Cref{fig:sketch} for a corresponding visualization. %\todoso{is it OK if i move Fig2 to be closer to this section? this whole section is essentially referring to fig2 right? if so, i can help stress this in the text itself}
We use notation from \cite{boumal2023introduction}, which provides a great introduction.



\paragraph{Linear embedding space} On the outer-most layer, we are given a linear Euclidean space $\gE \simeq \sR^d$ with $d$ the number of parameters.
We can think of $\gE$ as the \emph{computation space}.
For instance, for a loss function $\overline{\overline{\ell}}: \gE \to \sR, \vtheta \mapsto \overline{\overline{\ell}}(\vtheta)$ , we can use ML libraries to evaluate its value, as well as its Euclidean gradient
\begin{subequations}
  \begin{align}
    % \grad \overline{\overline{\ell}}: \gE \to \gE\,,
    % \quad
    % \vtheta \mapsto
    \grad_{\vtheta} \overline{\overline{\ell}}
    &=
      \left(
      \frac{\partial \overline{\overline{\ell}}(\vtheta)}{\partial \evtheta_i}
      \right)_{i=1,\dots, d} \in \sR^d
      \shortintertext{or Euclidean Hessian}
      % \hess \overline{\overline{\ell}}: \gE \to \sR^{d \times d}\,,
      % \quad
      % \vtheta \mapsto
      \hess_{\vtheta} \overline{\overline{\ell}}
    &=
      \left(
      \frac{\partial^2 \overline{\overline{\ell}}(\vtheta)}{\partial \evtheta_i \partial \evtheta_j}
      \right)_{i,j=1,\dots, d} \in \sR^{d\times d}\,.
  \end{align}
\end{subequations}
Because the geometry of $\gE$ is flat, i.e.\,uses the standard metric $\langle \vtheta_1, \vtheta_2 \rangle \coloneq \vtheta_1^{\top} \vtheta_2$, these objects consist of partial derivatives.
However, their Riemannian generalizations will add correction terms.

\paragraph{Total and quotient space} Into this computational space, we embed a sub-manifold $\overline{\gM}$ called the \emph{total space} and consider the restricted (loss) function $\overline{\ell} \coloneqq \overline{\overline{\ell}}\eval_{\overline{\gM}}: \overline{\gM} \to \sR$.
On that space, there is a symmetry in form of a group $\gG$ acting through an \emph{action} $\psi: \gG \times \overline{\gM} \to \overline{\gM}$ which transforms points in the total space to new points using a group element.
Let's further assume that $\overline{\ell}$ is symmetric under $\gG$, i.e.\,for any $x \in \overline{\gM}$ and all $g \in \gG$, $\overline{\ell}(x) = \overline{\ell}(\psi(g, x))$.

The symmetry imposes an equivalence relation $\sim$ on the total space: Two points $x, y \in \overline{\gM}$ are equivalent under the symmetry, if they can be mapped onto each other by the action,
\begin{align}
  x \sim y
  \quad \Leftrightarrow \quad
  \exists g \in \gG: y = \psi(g, x)\,.
\end{align}
In other words, if we let $\orbit(x) \coloneq \{ \psi(g, x) \mid g \in \gG \}$ be all points on the total space that are reachable from $x$ through the action of $\gG$, all points in an orbit are equivalent.
Instead of $\orbit(x)$, we will write
\begin{align}
  [x] \coloneq \{ y \in \overline{\gM} \mid y \sim x \}
\end{align}
for the symmetry-induced equivalence class $[x]$ of $x \in \overline{\gM}$.
This is an abstract object that lives in the \emph{quotient space}, $[x] \in \gM = \overline{\gM} / \gG$.
$\GL(h)$ is called a \emph{fiber space}.
If the action $\psi$ satisfies some technical conditions\footnote{See \cite{lee2003introduction} for more details.}, %\todoso{does this need a footnote?}, 
this quotient space is a Riemannian manifold called the \emph{Riemannian quotient manifold}.
The mapping between a point in total space to its equivalence class is called the \emph{natural projection}
\begin{align*}
  \pi: \overline{\gM} \to \gM, x \mapsto [x]\,.
\end{align*}
This leads to three perspectives of the original function $\overline{\overline{\ell}}$
\begin{itemize}[nosep]
\item In the Euclidean space: $\overline{\overline{\ell}}: \gE \to \sR, \vtheta \mapsto \overline{\overline{\ell}}(\vtheta)$

\item In the total space: $\overline{\ell}\coloneq \overline{\overline{\ell}}\eval_{\overline{\gM}} : \overline{\gM} \to \sR, x \mapsto \overline{\ell}(x)$

\item In the quotient space: $\ell \coloneq \overline{\ell} \circ \pi^{-1}:  \gM \to \sR, [x] \mapsto \ell([x]) = \overline{\ell}(\pi^{-1}(x))$
\end{itemize}

We would like to use the more sophisticated geometry of $\gM$ which treats all points in $\gM$ that are equivalent under the symmetry identically.
However, this comes at the cost of abstraction.
We cannot compute directly with objects on $\gM$ because points are equivalence classes, tangent vectors are equivalence classes of tangent vectors, and so on.
Our recipe will be to represent objects on $\gM$ by objects (on sub-spaces) on $\overline{\gM}$.
The key ingredient for doing so is the natural projection $\pi$ that establishes a connection between the total and quotient space.
This allows for computation in $\overline{\gM}$.
The concept we will use is called the \emph{horizontal lift}. %\todoso{overall this paragraph is great. note to self: i will think whether this is a good place to follow it up with a few more examples, or to put this paragraph a bit earlier on... or maybe just leave exactly as is, but highlight it in some way}

Manifold calculus on $\gM$ relies on the notion of the tangent space to a point $[x]$, denoted by $\mathrm{T}_{[x]}\gM$, which is a vector space that can be considered as the linearization of the non-linear manifold at that $[x]$.
Since the \emph{quotient manifold} $\gM$ is in principle abstract (in the sense that elements of $\gM$ are not immediately identified with matrices), the elements of its tangent space require a matrix representation in the total space $\overline{\gM}$ at $x$.
\mf{Look at this bit after restign a bit}
This matrix representation should respect the equivalence relationship $\sim$.
That is, the matrix representation of $\mathrm{T}_{[x]}\gM$ in $\overline{T}_x \overline{\gM}$ should be restricted to the directions that do not induce a displacement along the equivalence class $[x]$.

\paragraph{The horizontal space}
Our goal is to translate objects from the quotient space (tangent spaces/vectors, Riemannian gradients and Hessians) into computational representations in the total space.
These so-called \emph{horizontal lifts} do not cause displacements along symmetry directions, and are therefore identical for equivalent parameters in total space.

We can identify the so-called horizontal space containing all symmetry directions by considering the natural projection's differential $\mathrm{D}\pi$, and by using an appropriately defined metric, $\langle \cdot, \cdot \rangle_x$, on $\gM$. The directions along which $\pi$ does not change (the symmetry directions) are essentially uninteresting from the perspective of the quotient manifold, and we define the vertical space $\mathrm{V}_x \overline{\gM}$ as the kernel of $\mathrm{D}\pi$,
\begin{align}
  \mathrm{V}_x \overline{\gM}
  \coloneq
  % \ker \mathrm{D}\pi(x)
  % =
  \{ \xi \in \mathrm{T}_x \overline{\gM} \mid \mathrm{D}\pi(x)[\xi] = 0 \}
  \,.
\end{align}
Its orthogonal complement (w.r.t.\,$\langle \cdot, \cdot \rangle_x$) is the \emph{horizontal space} $\mathrm{H}_x \overline{\gM}$
\begin{align}
  \mathrm{H}_x \overline{\gM}
  =
  \{ \xi \in \mathrm{T}_x \overline{\gM} \mid \langle \xi, \eta \rangle_x = 0 \quad \forall \eta \in \mathrm{V}_x \overline{\gM} \}
  \,,
\end{align}
and the tangent space decomposes into vertical space and horizontal space (the orthogonal complement of the vertical space , $\mathrm{T}_x \overline{\gM} = \mathrm{H}_x \overline{\gM} \oplus \mathrm{V}_x \overline{\gM}$.
The horizontal space $\mathrm{H}_x \overline{\gM}$ is isomorphic to the tangent space $\mathrm{T}_{[x]} \gM$ on the quotient manifold.
We can therefore use it to represent an \emph{abstract} tangent vector on $\mathrm{T}_{[x]}\gM$ as a \emph{concrete} tangent vector in the horizontal space $\mathrm{T}_x \overline{\gM}$.
Conversely, we can decompose a tangent vector $\xi \in \mathrm{T}_x \overline{\gM}$ into its horizontal and vertical components $\xi^{\mathrm{H}} \in \mathrm{H}_x \overline{\gM}$ and $\xi^{\mathrm{V}} \in \mathrm{V}_x \overline{\gM}$,
\begin{align}
  \xi
  =
  \xi^{\mathrm{H}} + \xi^{\mathrm{V}} = \mathrm{Proj}^{\mathrm{H}}_x(\xi) + \mathrm{Proj}^{\mathrm{V}}_x(\xi)\,,
\end{align}
introducing the respective projectors.
The mapping $\mathrm{D}\pi(x) \eval_{\mathrm{H}_x \overline{\gM}}: \mathrm{H}_x \overline{\gM} \to \mathrm{T}_{[x]}\gM$ one-to-one.
It identifies a horizontal tangent vector with a tangent vector on the quotient manifold.
The inverse mapping $(\mathrm{D}\pi(x) \eval_{\mathrm{H}_x \overline{\gM}})^{-1}: \mathrm{T}_{[x]}\gM \to \mathrm{H}_x \overline{\gM}$ which maps a tangent vector $\xi_{[x]}$ on the quotient space with a tangent vector in the horizontal space is called the \emph{horizontal lift},
\begin{align}
  \lift_x(\xi_{[x]}) = \xi^{\mathrm{H}} \,.
\end{align}
It depends on the point $x \in \overline{\gM}$ we are lifting to.

The horizontal lift provides a means to work with tangent vectors on the quotient manifold $\gM$ through computations in the total space $\overline{\gM}$. The same concepts can be applied to vector fields, distances, gradients, connections, Hessians.

We can define a (Riemannian) metric on $\gM$ as:
\begin{align}
  \langle \xi_{[x]}, \zeta_{[x]} \rangle_{[x]}
  =
  \langle \lift_x(\xi_{[x]}), \lift_x(\zeta_{[x]}) \rangle_x
\end{align}
for some metric on $\overline{\gM}$, as long as  
\begin{align*}
x \sim y \implies \left\langle \text{lift}_x(\xi), \text{lift}_x(\zeta) \right\rangle_x = \left\langle \text{lift}_y(\xi), \text{lift}_y(\zeta) \right\rangle_y    
\end{align*}
This construction allows us to define Riemannian gradients on the quotient manifold as well. Let $f:\mathcal{M} \rightarrow \mathbb{R}$, then the Riemannian gradient $\operatorname{grad} f(x)$ is defined as the vector field that obeys
\begin{align*}
\mathrm{D} f(x)[v]=\langle v, \operatorname{grad} f(x)\rangle_x
\end{align*}
for all $v \in T_x \gM$ and all $x$. By considering the lift $\bar{f}=f \circ \pi$, one can show that
\begin{align*}
   \operatorname{lift}_x(\operatorname{grad} f([x]))=\operatorname{grad} \bar{f}(x) 
\end{align*}
Similarly, we can show that we have the following relation between the Hessian on the quotient manifold and the total space
\begin{align*}
    \operatorname{lift}_x(\operatorname{Hess} f([x])[\xi])=\operatorname{Proj}_x^{\mathrm{H}}(\operatorname{Hess} \bar{f}(x)[u])
\end{align*}
with $u=\operatorname{lift}_x(\xi)$.
\fd{Mention (i) Riemannian gradient and its lift, (ii) Riemannian connection and its lift,  (iii) Riemannian Hessian and its lift.} \mf{Seems good to you?}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/draft.tex <==
\newcommand{\Id}{\mathbbm{1}}
\def\argmax{\mathop{\rm arg\,max}}
\def\argmin{\mathop{\rm arg\,min}}
\def\argmaxop{\mathop{\rm arg\,max}\limits}
\def\argminop{\mathop{\rm arg\,min}\limits}
\def\minop{\mathop{\rm min}\limits}
\def\maxop{\mathop{\rm max}\limits}
\let\vec\relax
\newcommand{\vec}{\mathop{\rm vec}}
\newcommand{\sign}{\mathop{\rm sign}}
\def\R{\mathbb{R}}
\def\N{\mathbb{N}}
\def\U{\mathcal{U}}
\def\assign{\coloneqq}

\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\inner}[1]{\left\langle#1\right\rangle}
\newcommand*{\defeq}{\stackrel{\text{def}}{=}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand\eqdef{\ensuremath{\stackrel{\rm def}{=}}} %


\newcommand{\av}{\boldsymbol{a}}
\newcommand{\bv}{\boldsymbol{b}}
\newcommand{\cv}{\boldsymbol{c}}
\newcommand{\dv}{\boldsymbol{d}}
\newcommand{\ev}{\boldsymbol{e}}
\newcommand{\fv}{\boldsymbol{f}}
\newcommand{\gv}{\boldsymbol{g}}
\newcommand{\hv}{\boldsymbol{h}}
\newcommand{\iv}{\boldsymbol{i}}
\newcommand{\jv}{\boldsymbol{j}}
\newcommand{\kv}{\boldsymbol{k}}
\newcommand{\lv}{\boldsymbol{l}}
\newcommand{\mv}{\boldsymbol{m}}
\newcommand{\nv}{\boldsymbol{n}}
\newcommand{\ov}{\boldsymbol{o}}
\newcommand{\pv}{\boldsymbol{p}}
\newcommand{\qv}{\boldsymbol{q}}
\newcommand{\rv}{\boldsymbol{r}}
\newcommand{\sv}{\boldsymbol{s}}
\newcommand{\tv}{\boldsymbol{t}}
\newcommand{\uv}{\boldsymbol{u}}
\newcommand{\vv}{\boldsymbol{v}}
\newcommand{\wv}{\boldsymbol{w}}
\newcommand{\xv}{\boldsymbol{x}}
\newcommand{\yv}{\boldsymbol{y}}
\newcommand{\zv}{\boldsymbol{z}}

\newcommand{\Fv}{\boldsymbol{F}}
\newcommand{\Gv}{\boldsymbol{G}}

\newcommand{\vA}{\boldsymbol{A}}
\newcommand{\vB}{\boldsymbol{B}}
\newcommand{\vC}{\boldsymbol{C}}
\newcommand{\vD}{\boldsymbol{D}}
\newcommand{\vE}{\boldsymbol{E}}
\newcommand{\vF}{\boldsymbol{F}}
\newcommand{\vG}{\boldsymbol{G}}
\newcommand{\vH}{\boldsymbol{H}}
\newcommand{\vI}{\boldsymbol{I}}
\newcommand{\vJ}{\boldsymbol{J}}
\newcommand{\vK}{\boldsymbol{K}}
\newcommand{\vL}{\boldsymbol{L}}
\newcommand{\vM}{\boldsymbol{M}}
\newcommand{\vN}{\boldsymbol{N}}
\newcommand{\vO}{\boldsymbol{O}}
\newcommand{\vP}{\boldsymbol{P}}
\newcommand{\vQ}{\boldsymbol{Q}}
\newcommand{\vLambda}{\boldsymbol{\Lambda}}
\newcommand{\vR}{\boldsymbol{R}}
\newcommand{\vS}{\boldsymbol{S}}
\newcommand{\vT}{\boldsymbol{T}}
\newcommand{\vU}{\boldsymbol{U}}
\newcommand{\vV}{\boldsymbol{V}}
\newcommand{\vW}{\boldsymbol{W}}
\newcommand{\vX}{\boldsymbol{X}}
\newcommand{\vY}{\boldsymbol{Y}}
\newcommand{\vZ}{\boldsymbol{Z}}
\newcommand{\vTheta}{\boldsymbol{\Theta}}

\newcommand{\Xm}{\boldsymbol{X}}
\newcommand{\Ym}{\boldsymbol{Y}}
\newcommand{\Wm}{\boldsymbol{W}}

\newcommand{\Xmt}{\tilde{\Xm}}

\newcommand{\tr}{\text{tr}}
\newcommand{\lm}{\lambda_{\text{max}}}

\newcommand{\relu}{\text{ReLU}}
\newcommand{\gelu}{\text{GELU}}


\newcommand{\0}{\boldsymbol{0}}
\newcommand{\id}{\boldsymbol{\iota}}
\newcommand{\diag}{\mbox{$\mbox{diag}$}}
\newcommand{\bO}{\mathbb{O}}

\newcommand{\alphav}{\boldsymbol{\alpha}}
\newcommand{\betav}{\boldsymbol{\beta}}
\newcommand{\deltav}{\boldsymbol{\delta}}
\newcommand{\gammav}{\boldsymbol{\gamma}}
\newcommand{\thetav}{\boldsymbol{\theta}}
\newcommand{\muv}{\boldsymbol{\mu}}
\newcommand{\Sigmav}{\boldsymbol{\Sigma}}
\newcommand{\kappav}{\boldsymbol{\kappa}}
\newcommand{\phiv}{\boldsymbol{\phi}}
\newcommand{\piv}{\boldsymbol{\pi}}
\newcommand{\Phiv}{\boldsymbol{\Phi}}
\newcommand{\epsv}{\boldsymbol{\eps}}
\newcommand{\sigmav}{\boldsymbol{\sigma}}

\newcommand{\tvphi}{\widetilde{\phiv}}
\newcommand{\tvPhi}{\widetilde{\Phiv}}

\newcommand{\costfunc}{\mathcal{L}}
\newcommand{\deriv}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\secondderiv}[2]{\frac{\partial^2{#1}}{\partial{#2}^2}}



\newcommand{\Authornote}[2]{{\sffamily\small\color{red}{[#1: #2]}}}
\newcommand{\mnote}{\Authornote{MA}}

\newcommand{\MaxMnote}[2]{{\sffamily\small\color{purple}{[#1: #2]}}}
\newcommand{\maxmnote}{\MaxMnote{MM}}

\newcommand{\Maksymnote}[2]{{\sffamily\small\color{orange}{[#1: #2]}}}
\newcommand{\nf}{\Maksymnote{NF}}

\definecolor{darkgreen}{rgb}{0. .7 0.}
\newcommand{\fra}[1]{{\sffamily\small\color{darkgreen}{[Francesco: #1]}}}

\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Ncal}{\mathcal{N}}




\section{Experiments}



\section{Diagonal networks}

Here we look at a simple model/task: diagonal networks doing sparse regression.

Diagonal linear networks are defined as predictors  $\langle \xv, \betav\rangle$ with parameterization $\betav = \uv \odot \vv$ for weights $\wv = \left[\begin{smallmatrix}\uv\\\vv\end{smallmatrix}\right] \in \R^{2 d}$. 
We consider an overparametrized sparse regression problem for a data matrix $\vX \in \R^{n \times d}$ and label vector $\yv$:

\begin{align}\label{eq:dln_objective}
L(\wv) :=  \| \vX ( \uv \odot \vv) - \yv\|_2^2, 
\end{align}
for which the ground truth $\betav^*$ is a sparse vector and there exist many solutions $\wv$ such that $L(\wv)=0$.
\todofd{Meeting notes from June 17: The $\argmin_\vw \gL(\vw) = (\mX^\top \mX)^{-1} \mX^\top \vy$ in the diagonal network problem is unique under our assumptions on the data. This means that all minimizers $(\vv, \vu)$ belong to one equivalence class. Hence, if we were measuring flatness in a symmetry-agnostic manner, we would obtain the same value---which we do not if we use the modern look's sharpness metric.}
For now, we assume whitened data $\vX^\top \vX = \vI$ and that $\wv$ is a global minimum, so that the Hessian of the loss $L$ simplifies to 
\begin{align*}
\nabla^2 L(\wv) = 
\begin{bmatrix}
\diag(\vv \odot \vv) & \diag(\uv \odot \vv)  \\
\diag(\uv \odot \vv) & \diag(\uv \odot \uv)  
\end{bmatrix}.
\end{align*}
The average-case standard sharpness is equal to  $\tr(\nabla^2 L(\wv)) = \sum_{i=1}^d u_i^2 + v_i^2$ while the worst-case standard sharpness at a minimum is $\lm(\nabla^2 L(\wv)) = \maxop_{1 \leq i \leq d} v_i^2 + u_i^2$. 

Both average- and worst-case local sharpness are not invariant under $\alpha$-reparametrization $(\alpha \uv, \vv / \alpha)$ while the predictor $\betav=\uv\odot \vv$ is. \citep{andriushchenko2023modern}
use the carefully selected elementwise scaling $c_i = \sqrt{|v_i| / |u_i|} $ for $1 \leq i \leq d$ and $c_i = \sqrt{|u_i| / |v_i|}$ for $d < i \leq 2d$, obtaining for the average-case and worst-case adaptive local sharpness 
\begin{align*}
&S_{avg}^\rho(\wv, \cv) = \frac{1}{2} \!\sum_{i=1}^d\!u_i^2 |v_i| / |u_i| + \frac{1}{2}\!\sum_{i=1}^d\!v_i^2 |u_i| / |v_i| =\| \betav \|_1,\\ &S_{max}^\rho(\wv, \cv) = \maxop_{1 \leq i \leq d} |u_i| |v_i| = \| \betav \|_\infty.
\end{align*} 
Both definitions of adaptive sharpness are invariant under $\alpha$-reparametrization as they only depend on the predictor $\betav$. \citep{andriushchenko2023modern} notes that using $\cv = \wv$ in adaptive sharpness would instead lead to $\|\betav\|_2^2$ and $\|\betav\|_\infty^2$, so this scaling is clearly a hyper-parameter in these kinds of sharpness definitions.


To further illustrate this point, \citep{andriushchenko2023modern} train $200$ diagonal linear networks to $10^{-5}$ training loss on a sparse regression task ($d=200$ with $90\%$ sparsity) with different learning rates and random initializations. They find that, for example, the average-case adaptive sharpness correlates with generalization, while worst-case sharpness does not.

We start by trying to reproduce their results. 
\begin{figure}[H]
\begin{subfigure}{0.5\textwidth}
        \includegraphics[width=0.9\linewidth]{tex/paper/sections/draft/Initialization_simple_Savg.png}
        \caption{Average-case adaptive sharpness vs test loss}
    \end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \includegraphics[width=0.9\linewidth]{tex/paper/sections/draft/Initialization_simple_Smax.png}
    \caption{Worst-case adaptive sharpness vs test loss}
    \label{fig:enter-label}
\end{subfigure}
\end{figure}

This aren't quite the results from the Modern Look (worst-case sharpness roughly correlates, even if with a lower $\tau$), but there's an additional complication, that of scale of the parameters at initialisation. We now run the same experiments but with the neural network parameters being initially scaled by a $\sqrt{d}$ factor
\begin{figure}[H]
\begin{subfigure}{0.5\textwidth}
        \includegraphics[width=0.9\linewidth]{tex/paper/sections/draft/Initialization_complex_Savg.png}
        \caption{Average-case adaptive sharpness vs test loss}
    \end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \includegraphics[width=0.9\linewidth]{tex/paper/sections/draft/Initialization_complex_Smax.png}
    \caption{Worst-case adaptive sharpness vs test loss}
    \label{fig:enter-label}
\end{subfigure}
\end{figure}
Correlation between both sharpness measures and generalisation is completely lost. Note that even though the training losses are the same in both situations, the results from this smaller initialization are much flatter.

\todofd{Meeting notes from June 20: It might be that the outlier models correspond to poorly converged gradient ascents (getting stuck in some local maximum). To debug this, we should look at one of the outlier models, and try multiple restarts of the optimizer to see whether we can end up in other local maxima. Implement batches for toy model.}

\todomfs{Meeting notes from June 25: Run several restarts for all models.}

\section{Conclusion}
\input{sections/conclusion.tex}

\section{Timeline}

\begin{itemize}
    \item Week 0:
    \begin{itemize}
    \item Add sub-tasks to these big ticket items.
    \end{itemize}
    \item Week 1:
    \begin{itemize}
        \item Tuesday (Writing) 09/07/2024 - Clear structure for methods in place. Will take some re-organizing/moving things to appendix. Ideally, it would be all done, but at very least a clear structure should be defined. Felix suggestion: first explain things consistently, then optimize for space.
        \item Thursday (Research) 11/07/2024 - Toy model fully analysed (without data selection). 
    \end{itemize}
    \item Week 2:
    \begin{itemize}
        \item Tuesday (Writing) 16/07/2024 - Have the motivational subsection spelled out (consistent notation, references).  Some experimental discussion 
        \item Thursday (Research) 18/07/2024 - Role of data in toy model justified.  Fully understood, or at least significant progress in understanding, training dynamics for ImageNet models (second order possibly needed). Hopefully clear progress in outlier models.
    \end{itemize}
    \item Week 3:
    \begin{itemize}
        \item Tuesday (Writing) 23/07/2024 - Methods section writing completely done. Imagenet discussion done.
        \item Thursday (Research) 25/07/2024 -  Outlier models continuation if needed. Language models experiments starting
    \end{itemize}
    \item Week 4:
    \begin{itemize}
        \item Tuesday (Writing) 30/07/2024 - Experimental results fully discussed. Conclusions.
        \item Thursday (Research) 01/08/2024 - ImageNet fully done. Language models experiments either done or with significant progress.
    \end{itemize}
    \item Week 5:
    \begin{itemize}
        \item Tuesday (Writing) 06/08/2024 - Further refinements to paper.
        \item Thursday (Research) 01/08/2024 - All experiments done.
    \end{itemize}
\end{itemize}


==> sections/ideas.tex <==
\def\Hess{\mathop{\rm Hess}\nolimits}

% \subsection{Analysis of additional objects}
% \input{sections/additional_analysis_kunin.tex}

\paragraph{WIP (status: This does not solve the original goal of eliminating
  rotational symmetry):} We would like to eliminate this internal degree of
freedom by choosing a different functional form of the network. Since the output
depends only on the matrix-product $\mW^{(2)} \mW^{(1)} \in \sR^{n \times m}$,
we can pick any alternative parameterization for an $n\times m$ matrix.

Consider a singular-value decomposition parameterization $\vtheta = (\mW^{(1)},
\mW^{(2)}) \to \vpsi = (\mU^{(1)}, \mSigma^{(1)}, \mV^{(1)}, \mU^{(2)},
\mSigma^{(2)}, \mV^{(2)}) \in \sR^{h \times h} \times \sR^{h \times m} \times
\sR^{m\times m} \times \sR^{n \times n} \times \sR^{n \times h} \times \sR^{h
  \times h}$ and $f_{\vtheta}(\vx) \to f_{\vpsi}(\vx) = \mU^{(2)} \mSigma^{(2)}
{\mV^{(2)}}^{\top} \mU^{(1)} \mSigma^{(1)} {\mV^{(1)}}^{\top} \vx $. Notice that
we have the parameter constraints $\mU^{(i)} {\mU^{(i)}}^{\top}= \mI$,
$\mV^{(i)} {\mV^{(i)}}^{\top} = \mI$, and $\mSigma^{(i)}$ diagonal.

\subsection{Quotient manifold}
\subsubsection*{Toy problem}
We follow~\cite{edelman1998geometry}, while analyzing a two-layer neural network regression problem. We consider as inputs $x \in \mathbb{R}^n$, and targets $y \in \mathbb{R}$. We parametrize our network via the weight matrices $W, U$, which we restrict to be on the Stiefel manifolds $V_{p,n}$ and $V_{p,1}$, respectively, and where $p$ is the hidden dimension. $V_{p,n}=\{W \in \mathbb{R}^{p \times n}~|~W^T W = I_n \}$. We write our network as $F(x|U,W)= U^T W x$.

Given these definitions it is easy to see that if $Q \in O(p)$ is an orthogonal matrix, then, $U \rightarrow QU$ and $W \rightarrow QW$, leaves $F(\cdot | U, W)$ unchanged. \footnote{More generally, if $Q \in GL(n)$ is invertible, then $U \rightarrow QU$ and $W \rightarrow (Q^{-1})^T W$ then $F(\cdot | U, W)$ is also left unchanged, but we ignore this for now.}
\subsubsection{The Gradient of a Function (Grassmann)}

We must compute the gradient of a function $F(Y)$ defined on the
Grassmann manifold.  The
gradient of~$F$ at~$[Y]$ is defined to be the tangent vector
$\nabla F$ such that
\begin{equation}tr F_Y^T\Delta =g_c(\nabla
	F,\Delta) \equiv tr(\nabla F)^T\Delta
	\label{eq:grassgraddef}
	\end{equation} for~all tangent vectors
$\Delta$ at~$Y$, where $F_Y$ is defined by \begin{equation} (F_Y)_{ij}={\partial F\over \partial
		Y_{ij}}. \label{eq:FYdef} \end{equation}
Solving Eq.~(\ref{eq:grassgraddef}) for $\nabla F$ such that
$Y^T(\nabla F)=0$ yields \begin{equation} \nabla F = F_Y-YY^TF_Y.
	\label{eq:Gnpgradf}
\end{equation}


\subsubsection{The Hessian of a Function (Grassmann)}
\label{sec:GHess}
\begin{equation} \Hess F(\Delta,\Delta) =\left.{d^2\over
		dt^2}\right|_{t=0} F\bigl(Y(t)\bigr),
	\label{eq:Hessgdef}\end{equation} where $Y(t)$ is a geodesic
with tangent $\Delta$, i.e., $\dot Y(0)=\Delta$.

Applying the definition for the Hessian of~$F(Y)$ given by
Eq.~(\ref{eq:Hessgdef}) in the context of the Grassmann manifold yields
the formula \begin{equation} \Hess F(\Delta_1,\Delta_2) =
	F_{YY}(\Delta_1,\Delta_2) -tr(\Delta_1^T\Delta_2^T
	F_Y),\end{equation} where $F_Y$ is as in Eq.~(\ref{eq:FYdef}), and $F_{YY}$ is defined as $\sum_{ij,kl}
	(F_{YY})_{ij,kl}(\Delta_1)_{ij}(\Delta_2)_{kl}$, where \begin{equation}
	(F_{YY})_{ij,kl}={\partial^2 F\over \partial Y_{ij}\partial Y_{kl}}.
	\label{eq:FYYdef}\end{equation}

\paragraph{Long-term considerations}
\begin{itemize}

	\item Relation to pruning. Hessian eigenspectra are important to IMP (check out \cite{paul2022unmasking}), but we don't fully understand the impact that symmetries have on the eigenspectrum ({\color{red} At least I don't})
	\item How do discrete symmetries fit into the picture? In~\cite{ainsworth2022gitrebasin} permutation symmetries are used to remove loss barriers between minima. Can we do more?
	\item In \cite{kunin2021symmetry}, continuous symmetries are associated with conservation laws and impose restrictions on the model Hessian and gradient which has meaningful consequences for optimization. Can we do it in reverse, i.e. can we modify our architecture to do second-order optimization (or close to it) using only first-order methods by forcing an appropriate symmetry ({\color{red} Suspect not but leaving it here just in case the requisite symmetry doesn't disfigure our network too much})?
	\item Neural network symmetries can clearly be useful during optimization (as seen in \cite{zhao2023symmetry}), can we find a way to leverage this during optimization in a less ad hoc way (ideally we'd like to be doing optimization in a quotient manifold, M/G, where M is the standard parameter manifold, and G is our continuous symmetry manifold)?
    \item \so{not sure about this, but: is a slightly more complicated ``toy'' case to look at a possibly small 2-layer network where, e.g. one of the hidden units uses ReLU, and see how this causes a few different "cases" that need to be analyzed, i.e. regions where the prev analysis holds, and other regions where we can't apply it.. though i guess this might still require dealing with the non-invertible case...}
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/preliminaries.tex <==
%\todoso{COMPLETE THIS SECTION BY THURSDAY EVENING. NEEDS TO BE REFINED AND INTEGRATED INTO/WITH THE PREVIOUS/NEXT SECTION. NOTATION NEEDS TO BE DONE.}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

